Private delegated computations using strong isolation

Sensitive computations are now routinely delegated to third-parties. In response, Confidential Computing technologies are being introduced to microprocessors, offering a protected processing environment, which we generically call an isolate, providing confidentiality and integrity guarantees to code and data hosted within -- even in the face of a privileged attacker. Isolates, with an attestation protocol, permit remote third-parties to establish a trusted "beachhead" containing known code and data on an otherwise untrusted machine. Yet, the rise of these technologies introduces many new problems, including: how to ease provisioning of computations safely into isolates; how to develop distributed systems spanning multiple classes of isolate; and what to do about the billions of "legacy" devices without support for Confidential Computing? Tackling the problems above, we introduce Veracruz, a framework that eases the design and implementation of complex privacy-preserving, collaborative, delegated computations among a group of mutually mistrusting principals. Veracruz supports multiple isolation technologies and provides a common programming model and attestation protocol across all of them, smoothing deployment of delegated computations over supported technologies. We demonstrate Veracruz in operation, on private in-cloud object detection on encrypted video streaming from a video camera. In addition to supporting hardware-backed isolates -- like AWS Nitro Enclaves and Arm Confidential Computing Architecture Realms -- Veracruz also provides pragmatic "software isolates" on Armv8-A devices without hardware Confidential Computing capability, using the high-assurance seL4 microkernel and our IceCap framework.

==> evaluation/old_files/fs-read.tex <==
%\newcommand{\mibs}[1]{((67108864/\thisrow{#1})/1024/1024)}
\begin{tikzpicture}
\begin{axis} [
    width=\columnwidth * 0.4, height=3cm, %change figure dimensions
    %grid=both,
    ymajorgrids=true,
    %yminorgrids=true,
    grid style=dashed,
    align=center,
    ybar=1pt, %space between consecutive bars
    %xmin=0,
    ymin=0,
    axis y line*=none, axis x line*=none,
    bar width = 0.15cm,
    xtick = data,
    symbolic x coords={
        inorder,
        random,
    }, %allows to position coordinates on top of the bars
    x tick label style={rotate=60,anchor=east,font=\scriptsize},
    y tick label style={font=\scriptsize},
    nodes near coords,
    nodes near coords align={right},
    nodes near coords style={rotate=90, yshift=0.0cm, xshift=-0.05cm, font=\tiny, /pgf/number format/.cd,fixed zerofill,precision=2},
    %nodes near coords style={rotate=90, yshift=-0.2cm, xshift=0.5cm},
    point meta=rawy, % transform coordinates into log coordinates
    %mark options={rotate=180},
    legend pos=north west,
    legend style={
        inner xsep=0pt,inner ysep=20pt,nodes={inner xsep=3pt},
        legend columns=1,
        anchor=south west,
        draw=none,
        fill=none,
        font=\tiny,
        },
    enlarge x limits={rel=0.5},
    legend cell align=left,
    xlabel style={yshift=0.0cm},
    ylabel style={yshift=-0.1cm, font=\scriptsize},
    ylabel={MiB/s},
    area legend] 
]

\addplot [black,fill=arm-blue, postaction={pattern = north east lines}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{r-wt}, y error minus expr=\mibs{r-wt}-\mibs{r-wt-l}, y error plus expr=\mibs{r-wt-u}-\mibs{r-wt}] {evaluation/fs.txt}; 
%\addlegendentry[]{wasmtime};
\addplot [black,fill=arm-green, postaction={pattern = none}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{r-v-copy}, y error minus expr=\mibs{r-v-copy}-\mibs{r-v-copy-l}, y error plus expr=\mibs{r-v-copy-u}-\mibs{r-v-copy}] {evaluation/fs.txt};
%\addlegendentry[]{veracruz copy};
\addplot [black,fill=arm-orange, postaction={pattern = north west lines}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{r-v-no}, y error minus expr=\mibs{r-v-no}-\mibs{r-v-no-l}, y error plus expr=\mibs{r-v-no-u}-\mibs{r-v-no}] {evaluation/fs.txt};
%\addlegendentry[]{veracruz no-copy};
\addplot [black,fill=arm-grey, postaction={pattern = dots}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{r-soo}, y error minus expr=\mibs{r-soo}-\mibs{r-soo-l}, y error plus expr=\mibs{r-soo-u}-\mibs{r-soo}] {evaluation/fs.txt}; 
%\addlegendentry[]{veracruz soo};
\end{axis}

\end{tikzpicture}


==> evaluation/old_files/fs-update.tex <==
%\newcommand{\mibs}[1]{((67108864/\thisrow{#1})/1024/1024)}
\begin{tikzpicture}
\begin{axis} [
    width=\columnwidth * 0.4, height=3cm, %change figure dimensions
    %grid=both,
    ymajorgrids=true,
    %yminorgrids=true,
    grid style=dashed,
    align=center,
    ybar=1pt, %space between consecutive bars
    %xmin=0,
    ymin=0,
    axis y line*=none, axis x line*=none,
    bar width = 0.15cm,
    xtick = data,
    symbolic x coords={
        inorder,
        random,
    }, %allows to position coordinates on top of the bars
    x tick label style={rotate=60,anchor=east,font=\scriptsize},
    y tick label style={font=\scriptsize},
    nodes near coords,
    nodes near coords align={right},
    nodes near coords style={rotate=90, yshift=0.0cm, xshift=-0.05cm, font=\tiny, /pgf/number format/.cd,fixed zerofill,precision=2},
    %nodes near coords style={rotate=90, yshift=-0.2cm, xshift=0.5cm},
    point meta=rawy, % transform coordinates into log coordinates
    %mark options={rotate=180},
    legend pos=north west,
    legend style={
        inner xsep=0pt,inner ysep=20pt,nodes={inner xsep=3pt},
        legend columns=1,
        anchor=south west,
        draw=none,
        fill=none,
        font=\tiny,
        },
    enlarge x limits={rel=0.5},
    legend cell align=left,
    xlabel style={yshift=0.0cm},
    ylabel style={yshift=-0.1cm, font=\scriptsize},
    %ylabel={MiB/s},
    area legend] 
]

\addplot [black,fill=arm-blue, postaction={pattern = north east lines}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{u-wt}, y error minus expr=\mibs{u-wt}-\mibs{u-wt-l}, y error plus expr=\mibs{u-wt-u}-\mibs{u-wt}] {evaluation/fs.txt}; 
%\addlegendentry[]{wasmtime};
\addplot [black,fill=arm-green, postaction={pattern = none}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{u-v-copy}, y error minus expr=\mibs{u-v-copy}-\mibs{u-v-copy-l}, y error plus expr=\mibs{u-v-copy-u}-\mibs{u-v-copy}] {evaluation/fs.txt};
%\addlegendentry[]{veracruz copy};
\addplot [black,fill=arm-orange, postaction={pattern = north west lines}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{u-v-no}, y error minus expr=\mibs{u-v-no}-\mibs{u-v-no-l}, y error plus expr=\mibs{u-v-no-u}-\mibs{u-v-no}] {evaluation/fs.txt};
%\addlegendentry[]{veracruz no-copy};
\addplot [black,fill=arm-grey, postaction={pattern = dots}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{u-soo}, y error minus expr=\mibs{u-soo}-\mibs{u-soo-l}, y error plus expr=\mibs{u-soo-u}-\mibs{u-soo}] {evaluation/fs.txt}; 
%\addlegendentry[]{veracruz soo};
\end{axis}

\end{tikzpicture}


==> evaluation/old_files/fs-write.tex <==
\begin{tikzpicture}
\begin{axis} [
    width=\columnwidth * 0.4, height=3cm, %change figure dimensions
    %grid=both,
    ymajorgrids=true,
    %yminorgrids=true,
    grid style=dashed,
    align=center,
    ybar=1pt, %space between consecutive bars
    %xmin=0,
    ymin=0,
    axis y line*=none, axis x line*=none,
    bar width = 0.15cm,
    xtick = data,
    symbolic x coords={
        inorder,
        random,
    }, %allows to position coordinates on top of the bars
    x tick label style={rotate=60,anchor=east,font=\scriptsize},
    y tick label style={font=\scriptsize},
    nodes near coords,
    nodes near coords align={right},
    nodes near coords style={rotate=90, yshift=0.0cm, xshift=-0.05cm, font=\tiny, /pgf/number format/.cd,fixed zerofill,precision=2},
    %nodes near coords style={rotate=90, yshift=-0.2cm, xshift=0.5cm},
    point meta=rawy, % transform coordinates into log coordinates
    %mark options={rotate=180},
    legend pos=north west,
    legend style={
        inner xsep=0pt,inner ysep=10pt,nodes={inner xsep=3pt},
        legend columns=4,
        anchor=south,
        draw=none,
        fill=none,
        font=\tiny,
        at= {(current axis.north)}
        },
    enlarge x limits={rel=0.5},
    legend cell align=left,
    xlabel style={yshift=0.0cm},
    ylabel style={yshift=-0.1cm, font=\scriptsize},
    %ylabel={MiB/s},
    area legend] 
]

\addplot [black,fill=arm-blue, postaction={pattern = north east lines}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{w-wt}, y error minus expr=\mibs{w-wt}-\mibs{w-wt-l}, y error plus expr=\mibs{w-wt-u}-\mibs{w-wt}] {evaluation/fs.txt}; 
\addlegendentry[]{tmpfs};
\addplot [black,fill=arm-green, postaction={pattern = none}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{w-v-copy}, y error minus expr=\mibs{w-v-copy}-\mibs{w-v-copy-l}, y error plus expr=\mibs{w-v-copy-u}-\mibs{w-v-copy}] {evaluation/fs.txt};
\addlegendentry[]{Veracruz copy};
\addplot [black,fill=arm-orange, postaction={pattern = north west lines}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{w-v-no}, y error minus expr=\mibs{w-v-no}-\mibs{w-v-no-l}, y error plus expr=\mibs{w-v-no-u}-\mibs{w-v-no}] {evaluation/fs.txt};
\addlegendentry[]{Veracruz no-copy};
\addplot [black,fill=arm-grey, postaction={pattern = dots}, error bars/.cd, y dir=both, y explicit] table[skip first n=1, x=name, y expr=\mibs{w-soo}, y error minus expr=\mibs{w-soo}-\mibs{w-soo-l}, y error plus expr=\mibs{w-soo-u}-\mibs{w-soo}] {evaluation/fs.txt}; 
\addlegendentry[]{Veracruz\\no-copy+soo};
\end{axis}
\end{tikzpicture}


==> figs/tree_of_certs.tex <==
\begin{tikzpicture}[font=\footnotesize]
\node[align=center, draw] (root) {Root Proxy\\Certificate};
\node[align=center, draw] (a) at ($(root.south)-(1.2,1)$) {Target Profile A\\Certificate};
\node[align=center, draw] (b) at ($(root.south)-(-1.2,1)$) {Target Profile B\\Certificate};
\node[align=center, draw] (aa) at ($(a.south)-(2.5,1)$) {Target Profile AA\\Certificate};
\node[align=center, draw] (ab) at ($(a.south)-(0,1)$) {Target Profile AB\\Certificate};
\node[align=center, draw] (ba) at ($(b.south)-(0,1)$) {Target Profile BA\\Certificate};
\node[align=center] (dots) at ($(b.south)-(-2,1)$) {...};

\coordinate (mid-a-b) at ($(a)!0.5!(b)$);
\coordinate (mid-a-b-root) at ($(mid-a-b)!0.5!(root)$);
\coordinate (mid-a-ab) at ($(a)!0.5!(ab)$);
\coordinate (mid-b-ba) at ($(b)!0.5!(ba)$);

\draw[-Latex] (root) -- (mid-a-b-root) -| (a.north);
\draw[-Latex] (root) -- (mid-a-b-root) -| (b.north);
\draw[-Latex] (a) -- (mid-a-ab) -- (ab);
\draw[-Latex] (a) -- (mid-a-ab) -| (aa);
\draw[-Latex] (b) -- (ba);
\draw[-Latex] (b) -- (mid-b-ba) -| (dots);

\end{tikzpicture}


==> s4.5-veracruz-e2e-deployment.tex <==


